Marital Stability With Committed Couples: A Revealed Preference Analysis

We present a revealed preference characterization of marital stability where some couples are committed. A couple is committed if they can divorce only with mutual consent. We provide theoretical insights into the potential of the characterization for identifying intrahousehold consumption patterns. We demonstrate that without price variation for private goods among potential couples, intrahousehold resource allocations can only be identified for non-committed couples. We conduct simulations using Dutch household data to support our theoretical findings. Our results show that with price variation, the empirical implications of marital stability allow for the identification of household consumption allocations for both committed and non-committed couples.

==> tables/DivorceCosts_full.tex <==
%\begin{landscape}
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcHcHcHcHcHc}
\toprule
%\multicolumn{12}{l}{{\it Panel A: prices}} \\ \midrule
                                              & 0\%                                                         & 5\%                                                         & 10\%                                                        & 15\%                                                        & 20\%                                                        & 25\%                                                        & 30\%                                                        & 35\%                                                        & 40\%                                                          & 45\%                                                          & 50\%                                                          \\ \midrule
{\it Panel A: prices}    &  &   &  &  & & & & & &  & \\ 
%\midrule
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.9995\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9994\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9992\\ \footnotesize .95 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9990\\ \footnotesize .95 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9985\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9981\\ \footnotesize .93 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9975\\ \footnotesize .93 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9969\\ \footnotesize .92 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9963\\ \footnotesize .91 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9955\\ \footnotesize .90 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9947\\ \footnotesize .89 1 1 1 1\end{tabular}   \\
\multicolumn{1}{l}{mutual consent w/o transfers}                
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .95 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}         \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       & \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .99 1 1 1 1\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9996\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9993\\ \footnotesize .96 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9989\\ \footnotesize .95 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9984\\ \footnotesize  94 1 1 1 1\end{tabular}  & \begin{tabular}[c]{@{}c@{}}.9979\\ \footnotesize .93 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9971\\ \footnotesize .91 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9965\\ \footnotesize .87 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9958\\ \footnotesize .89 1 1 1 1\end{tabular}   \\ \midrule
                                                 %  \multicolumn{12}{l}{{\it Panel B: Wages}}                       \\ \hline%{\it Panel B: wages}    & 0\%                                                         & 5\%                                                         & 10\%                                                        & 15\%                                                        & 20\%                                                        & 25\%                                                        & 30\%                                                        & 35\%                                                        & 40\%                                                          & 45\%                                                          & 50\%                                   \\ \hline
                                                 {\it Panel B: wages}    &  &   &  &  & & & & & &  & \\ 
                                                 %\midrule
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.9995\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9994\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9991\\ \footnotesize .95 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9988\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9983\\ \footnotesize .92 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9978\\ \footnotesize .91 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9971\\ \footnotesize .90 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9964\\ \footnotesize .88 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9958\\ \footnotesize .87 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9949\\ \footnotesize .87 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9941\\ \footnotesize .85 .99 1 1 1\end{tabular} \\
\multicolumn{1}{l}{mutual consent w/o transfers}                
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .99 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .99 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .96 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .96 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .94 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .95 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .95 1 1 1 1\end{tabular}         \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       & \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .99 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9998\\ \footnotesize .98 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9995\\ \footnotesize .96 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9990\\ \footnotesize .96 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9985\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9978\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9971\\ \footnotesize .92 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9964\\ \footnotesize .92 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9955\\ \footnotesize .91 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9948\\ \footnotesize .90 1 1 1 1\end{tabular}   \\ \midrule
                                                  % \multicolumn{12}{l}{{\it Panel C: prices and wages}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
            %                             {\it Panel C: prices and wages}          & 0\%                                                         & 5\%                                                         & 10\%                                                        & 15\%                                                        & 20\%                                                        & 25\%                                                        & 30\%                                                        & 35\%                                                        & 40\%                                                          & 45\%                                                          & 50\%                                                          \\ 
    {\it Panel C: prices and wages}    &  &   &  &  & & & & & &  & \\ 
    %\midrule
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.9995\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9993\\ \footnotesize .96 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9989\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9983\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9975\\ \footnotesize .91 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9967\\ \footnotesize .90 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9956\\ \footnotesize .88 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9944\\ \footnotesize .86 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9933\\ \footnotesize .83 .99 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9919\\ \footnotesize .81 .99 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9906\\ \footnotesize .82 .99 1 1 1\end{tabular} \\
\multicolumn{1}{l}{mutual consent w/o transfers}                
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize  1 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize  .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .98 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .96 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .94 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .95 1 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .97 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .94 1 1 1 1\end{tabular}         
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}         \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1 1 1\end{tabular}       & \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .98 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9996\\ \footnotesize .97 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9991\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9983\\ \footnotesize .94 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9975\\ \footnotesize .92 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9965\\ \footnotesize .91 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9954\\ \footnotesize .88 1 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9942\\ \footnotesize .88 1 1 1 1\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.9930\\ \footnotesize .86 .99 1 1 1\end{tabular} & \begin{tabular}[c]{@{}c@{}}.9917\\ \footnotesize .86 .99 1 1 1\end{tabular} \\ \bottomrule
\end{tabular}
}
{
\\[0.2em]
\raggedright  \scriptsize {\it Notes:} The number in each cell is the mean value for the distribution of stability indices in the given scenario. The five numbers below correspond to the quartiles of the distribution: min, 25\%, 50\%, 75\%, max.
\par}
\caption{Stability indices}
\label{tab:ResultsDivorceCosts}
\end{table}
%\end{landscape}

==> tables/PassRates.tex <==
%\begin{landscape}
\begin{table}[htbp]
\centering
%\resizebox{\textwidth}{!}{
\begin{tabular}{lcHcHcHcHcHc}
\toprule
%\multicolumn{12}{l}{{\it Panel A: prices}} \\ \midrule
   & 0\%  & 5\%  & 5\%  & 15\%  & 10\%   & 25\%   & 15\% & 35\%  & 20\% & 45\%  & 25\% \\ \midrule
{\it Panel A: prices}    &  &   &  &  & & & & & &  & \\ 
%\midrule
unilateral                  
& 0 
& 0
& 0
& 0
& 0
& 0
& 0 
& 0
& 0
& 0
& 0 \\

mutual consent w/o transfers  
& 1
& 0.94  
& 0.93    
& 0.92     
& 0.95       
& 0.93     
& 0.97       
& 0.94    
& 0.99       
& 0.96      
& 0.96     \\

\multicolumn{1}{l}{mutual consent with transfers} 
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1\end{tabular}    
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize .99 1 1 1 1\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .97 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9996\\ \footnotesize .97 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9993\\ \footnotesize .96 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9989\\ \footnotesize .95 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9984\\ \footnotesize  94 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9979\\ \footnotesize .93 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9971\\ \footnotesize .91 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9965\\ \footnotesize .87 1 1 1 1\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}.9958\\ \footnotesize .89 1 1\end{tabular}   \\ \midrule
                                                 %  \multicolumn{12}{l}{{\it Panel B: Wages}}                       \\ \hline%{\it Panel B: wages}    & 0\%                                                         & 5\%                                                         & 10\%                                                        & 15\%                                                        & 20\%                                                        & 25\%                                                        & 30\%                                                        & 35\%                                                        & 40\%                                                          & 45\%                                                          & 50\%                                   \\ \hline
                                                 {\it Panel B: income}    &  &   &  &  & & & & & &  & \\ 
                                                 %\midrule
unilateral                    
& 0
& 0
& 0
& 0
& 0 
& 0 
& 0 
& 0 
& 0
& 0 
& 0 \\

mutual consent w/o transfers               
& 1   
& 0.99      
& 1.00
& 0.94      
& 0.96    
& 0.95      
& 0.89       
& 0.88      
& 0.91       
& 0.86         
& 0.87        \\

\multicolumn{1}{l}{mutual consent with transfers} 
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .99 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9998\\ \footnotesize .98 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9995\\ \footnotesize .96 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9990\\ \footnotesize .96 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9985\\ \footnotesize .94 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9978\\ \footnotesize .94 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9971\\ \footnotesize .92 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9964\\ \footnotesize .92 1 1\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}.9955\\ \footnotesize .91 1 1 1 1\end{tabular}  
& \begin{tabular}[c]{@{}c@{}}.9948\\ \footnotesize .90 1 1\end{tabular}   \\ \midrule
                                                  % \multicolumn{12}{l}{{\it Panel C: prices and wages}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
            %                             {\it Panel C: prices and wages}          & 0\%                                                         & 5\%                                                         & 10\%                                                        & 15\%                                                        & 20\%                                                        & 25\%                                                        & 30\%                                                        & 35\%                                                        & 40\%                                                          & 45\%                                                          & 50\%                                                          \\ 
    {\it Panel C: prices and income}    &  &   &  &  & & & & & &  & \\ 
    %\midrule
unilateral                    
& 0
& 0
& 0
& 0 
& 0
& 0 
& 0
& 0
& 0 
& 0 
& 0 \\

mutual consent w/o transfers     
& 1
& 0.93       
& 0.94      
& 0.95   
& 0.95     
& 0.95       
& 0.93      
& 0.91     
& 0.92  
& 0.97      
& 1.00         \\

\multicolumn{1}{l}{mutual consent with transfers} 
& \begin{tabular}[c]{@{}c@{}}1\\ \footnotesize 1 1 1\end{tabular}       
& \begin{tabular}[c]{@{}c@{}}.9999\\ \footnotesize .98 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9996\\ \footnotesize .97 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9991\\ \footnotesize .94 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9983\\ \footnotesize .94 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9975\\ \footnotesize .92 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9965\\ \footnotesize .91 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9954\\ \footnotesize .88 1 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9942\\ \footnotesize .88 1 1\end{tabular}   
& \begin{tabular}[c]{@{}c@{}}.9930\\ \footnotesize .86 .99 1 1 1\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}.9917\\ \footnotesize .86 1 1\end{tabular} \\ \bottomrule
\end{tabular}
%}
{
\\[0.2em]
\raggedright  \scriptsize {\it Notes:} The number in each cell is the pass rate of the model given the simulation scenario
\par}
\caption{Pass Rates}
\label{tab:ResultsDivorceCosts}
\end{table}
%\end{landscape}

==> tables/SharingRules_full.tex <==
%\begin{landscape}
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcHcHcHcHcHc}
\toprule
%                                                   & \multicolumn{11}{c}{Prices}                                                                                            \\ \hline
                                       & 0\%                                                                               & 5\%                                                                               & 10\%                                                                              & 15\%                                                                              & 20\%                                                                              & 25\%                                                                              & 30\%                                                                              & 35\%                                                                              & 40\%                                                                              & 45\%                                                                              & 50\%                                                                                       \\\midrule
                                            {\it Panel A: prices}       &&&&&&&&&&&\\
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.0869\\ \footnotesize 0 .02 .06 .12 .52\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.0036\\ \footnotesize 0 0 0 0 .54\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0008\\ \footnotesize 0 0 0 0 .14\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0002\\ \footnotesize 0 0 0 0 .11\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0003\\ \footnotesize 0 0 0 0 .53\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}           & \begin{tabular}[c]{@{}c@{}}.0001\\ \footnotesize 0 0 0 0 .36\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}           & \begin{tabular}[c]{@{}c@{}}.0001\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 .01 .45\end{tabular}       & \begin{tabular}[c]{@{}c@{}}.0001\\ \footnotesize 0 0 0 0 .29\end{tabular}                  \\
\multicolumn{1}{l}{mutual consent w/o transfers}                & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular}          \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.2643\\ \footnotesize 0 0 .09 .56 .84\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0985\\ \footnotesize 0 0 0 0 .84\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0642\\ \footnotesize 0 0 0 0 .83\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0384\\ \footnotesize 0 0 0 0 .63\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0272\\ \footnotesize 0 0 0 0 .63\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0165\\ \footnotesize 0 0 0 0 .63\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0108\\ \footnotesize 0 0 0 0 .56\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0085\\ \footnotesize 0 0 0 0 .56\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0051\\ \footnotesize 0 0 0 0 .49\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0036\\ \footnotesize 0 0 0 0 .56\end{tabular}                  \\ \midrule
%                                                   & \multicolumn{11}{c}{Wages}                                               \\ \hline
 {\it Panel B: wages}          &&&&&&&&&&&\\
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.0869\\ \footnotesize 0 .02 .06 .12 .52\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.0802\\ \footnotesize 0 .01 .05 .11 .59\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.0794\\ \footnotesize 0 .01 .05 .11 .63\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.0781\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0777\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0787\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0786\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0793\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0798\\ \footnotesize 0 0 .05 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0798\\ \footnotesize 0 0 .06 .11 .63\end{tabular}     & \begin{tabular}[c]{@{}c@{}}.0789\\ \footnotesize 0 0 .05 .11 .63\end{tabular}              \\
\multicolumn{1}{l}{mutual consent w/o transfers}                & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & {\begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular}} \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular}          \\ \midrule
%                                                   & \multicolumn{11}{c}{Prices and Wages}                                                                                                                                                     \\ \hline
 {\it Panel C: prices and wages}          &&&&&&&&&&&\\
\multicolumn{1}{l}{unilateral}                    & \begin{tabular}[c]{@{}c@{}}.0869\\ \footnotesize 0 .02 .06 .12 .52\end{tabular}   & \begin{tabular}[c]{@{}c@{}}.0019\\ \footnotesize 0 0 0 0 .56\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0006\\ \footnotesize 0 0 0 0 .39\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0003\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0005\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0003\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0001\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0001\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 .71\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 .16\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 .48\end{tabular}                  \\
\multicolumn{1}{l}{mutual consent w/o transfers}                & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular}          \\
\multicolumn{1}{l}{mutual consent with transfers} & \begin{tabular}[c]{@{}c@{}}.6070\\ \footnotesize .24 .55 .61 .69 .84\end{tabular} & \begin{tabular}[c]{@{}c@{}}.1218\\ \footnotesize 0 0 0 .12 .84\end{tabular}       & \begin{tabular}[c]{@{}c@{}}.0347\\ \footnotesize 0 0 0 0 .82\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0151\\ \footnotesize 0 0 0 0 .63\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0040\\ \footnotesize 0 0 0 0 .56\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0012\\ \footnotesize 0 0 0 0 .56\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0002\\ \footnotesize 0 0 0 0 .24\end{tabular}         & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}           & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}           & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}           & \begin{tabular}[c]{@{}c@{}}.0000\\ \footnotesize 0 0 0 0 0\end{tabular}       
\\ \bottomrule
\end{tabular}
}
{
\\[0.3em]
\raggedright  \scriptsize {\it Notes:} The number in each cell is the mean value of the difference between upper and lower bounds on female private consumption shares in the given scenario. The five numbers below correspond to the quartiles of the distribution: min, 25\%, 50\%, 75\%, max. 
\par}
\caption{Intrahousehold identification}
\label{tab:SharingRuleResults}
\end{table}
%\end{landscape}
